LLM-PS: Empowering Large Language Models for Time Series Forecasting with Temporal Patterns and Semantics

Time Series Forecasting (TSF) is critical in many real-world domains like financial planning and health monitoring. Recent studies have revealed that Large Language Models (LLMs), with their powerful in-contextual modeling capabilities, hold significant potential for TSF. However, existing LLM-based methods usually perform suboptimally because they neglect the inherent characteristics of time series data. Unlike the textual data used in LLM pre-training, the time series data is semantically sparse and comprises distinctive temporal patterns. To address this problem, we propose LLM-PS to empower the LLM for TSF by learning the fundamental \textit{Patterns} and meaningful \textit{Semantics} from time series data. Our LLM-PS incorporates a new multi-scale convolutional neural network adept at capturing both short-term fluctuations and long-term trends within the time series. Meanwhile, we introduce a time-to-text module for extracting valuable semantics across continuous time intervals rather than isolated time points. By integrating these patterns and semantics, LLM-PS effectively models temporal dependencies, enabling a deep comprehension of time series and delivering accurate forecasts. Intensive experimental results demonstrate that LLM-PS achieves state-of-the-art performance in both short- and long-term forecasting tasks, as well as in few- and zero-shot settings.

==> sec/alg.tex <==
\begin{algorithm}
	\caption{LLM-PS for Time Series Forecasting}
	\label{alg:llmps}
	\begin{algorithmic}[1]
		\REQUIRE Historical time series data $\mathbf{X} \in \mathbb{R}^{H \times V}$, prediction horizon $T$
		\ENSURE Forecasted time series $\hat{\mathbf{Y}} \in \mathbb{R}^{T \times V}$
		\STATE \textbf{Step 1: Multi-Scale Features Extraction (MSCNN)}
		\STATE Initialize $B$ parallel branches with varying receptive fields
		\FOR{$i \gets 1$ to $B$}
		\IF{$i = 1$}
		\STATE $\bar{F}_i \gets \text{Conv}_i(F_i)$
		\ELSE
		\STATE $\bar{F}_i \gets \text{Conv}_i(F_i + \bar{F}_{i-1})$
		\ENDIF
		\ENDFOR
		\STATE Concatenate features $\{\bar{F}_1, \dots, \bar{F}_B\}$ and fuse via a $1 \times 1$ convolution:
		\STATE $F_{\text{out}} \gets \text{Conv}_{1\times1}(\text{Concat}(\{\bar{F}_1, \dots, \bar{F}_B\}) + F_{\text{in}})$
		
		\STATE \textbf{Step 2: Temporal Patterns Decoupling and Assembling}
		\STATE Decouple $F_{\text{out}}$ into low- and high-frequency components:
		\STATE $W_{\text{low}}, W_{\text{high}} \gets \text{WT}(F_{\text{out}})$
		\STATE Construct short-term and long-term patterns:
		\STATE $P_S \gets \text{IWT}(\text{Zero}(W_{\text{low}}), W_{\text{high}})$
		\STATE $P_L \gets \text{IWT}(W_{\text{low}}, \text{Zero}(W_{\text{high}}))$
		\FOR{$b \gets 1$ to $B$}
		\STATE $P_S^b \gets P_S^b + P_S^{b-1}$
		\ENDFOR
		\FOR{$b \gets B-1$ to $0$ (decreasing order)}
		\STATE $P_L^b \gets P_L^b + P_L^{b+1}$
		\ENDFOR
		\STATE Reconstruct features: $\bar{F}_b \gets P_S^b + P_L^b$ for all $b$
		
		\STATE \textbf{Step 3: Time-to-Text (T2T) Semantics Extraction}
		\STATE Divide $X$ into $P$ patches $\{X_i\}_{i=1}^P$, where $X_i \in \mathbb{R}^{L \times V}$
		\STATE Randomly mask $75\%$ of the patches
		\STATE Train T2T by minimizing:
		\STATE $L_{\text{T2T}} \gets \frac{1}{P} \sum_{i=1}^P \left( 1[M(i)=1] \| X_i - \hat{X}_i \|^2 + l_i \log \frac{l_i}{\hat{l}_i} \right)$
		
		\STATE \textbf{Step 4: Integration and Forecasting}
		\STATE Integrate $F_{\text{MSCNN}}$ and $F_{\text{T2T}}$ via feature transfer
		\STATE Input combined features into LLM for forecasting
		\STATE Minimize overall loss:
		\STATE $L_{\text{OBJ}} \gets L_{\text{TIME}} + \lambda L_{\text{FEAT}}$
		\STATE where:
		\STATE $L_{\text{TIME}} \gets \frac{1}{T} \sum_{i=1}^T \| Y_i - \hat{Y}_i \|^2$
		\STATE $L_{\text{FEAT}} \gets \frac{1}{C} \sum_{j=1}^C \| F_j^{\text{MSCNN}} - F_j^{\text{T2T}} \|^2$`
		
	\end{algorithmic}
\end{algorithm}

==> table/stf.tex <==
\begin{table*}[ht]
	\caption{Average results of short-term forecasting in monthly, quarterly, yearly, and others. The input and output time series lengths are $[12, 96]$ and $[6, 48]$, respectively.  Tab.~\ref{tab::short-term_appendix} reports the full results.}
	\label{tab::short-term}
	\setlength{\tabcolsep}{3.5pt}
	\tiny
	\centering
	\begin{threeparttable}
		\begin{tabular}{cc|ccccccccccccccc}
			\toprule
			
			\multicolumn{2}{c}{\multirow{1}{*}{\scalebox{1.1}{Models}}}&LLM-PS & CALF & TimeLLM & GPT4TS & PatchTST & iTransformer & ETSformer & FEDformer & Autoformer & TimesNet & TCN & N-HiTS & N-BEATS & DLinear & TimeMixer \\ 
			\multicolumn{2}{c}{} & \scalebox{0.8}{(\textbf{Ours})} &
			\scalebox{0.8}{\citeyearpar{liu2024taming}} &
			 \scalebox{0.8}{\citeyearpar{jintime}} & \scalebox{0.8}{\citeyearpar{zhou2023onefitsall}} & \scalebox{0.8}{\citeyearpar{nie2022pathtst}} & \scalebox{0.8}{\citeyearpar{liu2023itransformer}}& \scalebox{0.8}{\citeyearpar{woo2022etsformer}} & \scalebox{0.8}{\citeyearpar{zhou2022fedformer}} & \scalebox{0.8}{\citeyearpar{wu2021autoformer}} & \scalebox{0.8}{\citeyearpar{wu2023timesnet}} & \scalebox{0.8}{\citeyearpar{BaiTCN2018}} & \scalebox{0.8}{\citeyearpar{challu2022nhits}} & \scalebox{0.8}{\citeyearpar{oreshkin2019nbeats}} & \scalebox{0.8}{\citeyearpar{zeng2023dlinear}}  & \scalebox{0.8}{\citeyearpar{wangtimemixer}} \\
			
			\toprule
			
			\multirow{3}{*}{\rotatebox[origin=c]{90}{\scalebox{0.8}{Average}}}
			
			& \scalebox{0.8}{SMAPE} &\best{11.708} & \second{11.770} & 11.983 & 11.991 & 12.059 &12.726 & 14.718 & 12.840 & 12.909 & 11.829 & 13.961 & 11.927 & 11.851 & 13.639 &11.784 \\
			
			& \scalebox{0.8}{MASE}&\best{1.557}  & \second{1.570}  & 1.595 & 1.600  & 1.623  &1.761 & 2.408  & 1.701  & 1.771  & 1.585  & 1.945  & 1.613  & 1.599  & 2.095  &1.574  \\
			
			& \scalebox{0.8}{OWA} &\best{0.839} & \second{0.845}  & 0.859 & 0.861  & 0.869  &0.929 & 1.172  & 0.918  & 0.939  & 0.851  & 1.023  & 0.861  & 0.855  & 1.051 &0.850  \\
			\midrule
			\multicolumn{2}{c|}{$1^{\text{st}}$ \emph{Count}} & \multicolumn{1}{c}{\best{3}}& \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{0}\\	
			
			\bottomrule
			
		\end{tabular}
	\end{threeparttable}
\end{table*}
